Inverse regression for spatially distributed functional data

Spatially distributed functional data are prevalent in many statistical applications such as meteorology, energy forecasting, census data, disease mapping, and neurological studies. Given their complex and high-dimensional nature, functional data often require dimension reduction methods to extract meaningful information. Inverse regression is one such approach that has become very popular in the past two decades. We study the inverse regression in the framework of functional data observed at irregularly positioned spatial sites. The functional predictor is the sum of a spatially dependent functional effect and a spatially independent functional nugget effect, while the relation between the scalar response and the functional predictor is modeled using the inverse regression framework. For estimation, we consider local linear smoothing with a general weighting scheme, which includes as special cases the schemes under which equal weights are assigned to each observation or to each subject. This framework enables us to present the asymptotic results for different types of sampling plans over time such as non-dense, dense, and ultra-dense. We discuss the domain-expanding infill (DEI) framework for spatial asymptotics, which is a mix of the traditional expanding domain and infill frameworks. The DEI framework overcomes the limitations of traditional spatial asymptotics in the existing literature. Under this unified framework, we develop asymptotic theory and identify conditions that are necessary for the estimated eigen-directions to achieve optimal rates of convergence. Our asymptotic results include pointwise and $L_2$ convergence rates. Simulation studies using synthetic data and an application to a real-world dataset confirm the effectiveness of our methods.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> localdef.tex <==

newcommand{xmark}{textrm{ding{53}}}%
%usepackage{cite}
%usepackage{booktabs,caption,fixltx2e}
usepackage{threeparttable}
newenvironment{resp}
{begin{quotation}% 
noindent AUTHORS%
it}%
{end{quotation}}
topmargin=-0.1in
oddsidemargin=0.1in evensidemargin=0.1in textwidth=6.4in
textheight=8.8in
usepackage[normalem]{ulem}
defshang{textcolor{red}}
defLTR{L^2(bbR)}
defbbR{mathbb{R}}
defbbZ{mathbb{Z}}
defbbN{mathbb{N}}
defP{mathsf{P}}
def mcF{mathcal{F}}
def mcFn{mathcal{F}_n}
def mcH{mathcal{H}}
def mcX{mathcal{X}}
def mcC{mathcal{C}}
def mcE{mathcal{E}}
def mcCS{mathcal{C}mathcal{S}}
def mcG{mathcal{G}}
def mcD{mathcal{D}}
def mcRn{mathcal{R}_n}
def mbI{mathbb{I}}
def mcR{mathcal{R}}
def mcB{mathcal{B}}
def mcN{mathcal{N}}
def mcP{mathcal{P}}
def mcV{mathcal{V}}
def mcS{mathcal{S}}
def mcNN{mathcal{N}mathcal{N}}
def whb{widehat{beta}}
def wha{widehat{alpha}}
def udb{underline{beta}}
def bfgamma{bm{gamma}}

defliu{textcolor{red}}



newcommand{Argmax}{mathop{mathrm{argmax}}}  
newcommand{Argmin}{mathop{mathrm{argmin}}}  
def cov{textrm{cov}}
def mcNN{mathcal{N}mathcal{N}}
def mcA{mathcal{A}}
def bfx{mathbf{x}}
def bfs{mathbf{s}}
def bfD{mathbf{D}}
def bfg{mathbf{g}}
def bfX{mathbf{X}}
def bfx{mathbf{x}}
def bfsigma{bm{sigma}}
def bfZ{mathbf{Z}}
def bfz{mathbf{z}}
def bfd{mathbf{d}}
def bft{mathbf{t}}
def bfh{mathbf{h}}
def bfp{mathbf{p}}
def bfV{mathbf{V}}
def bfa{mathbf{a}}
def bftheta{bm{theta}}
def bfb{mathbf{b}}
def bfy{mathbf{y}}
def bfD{mathbf{D}}
def bfB{mathbf{B}}
def bfY{mathbf{Y}}
def bff{mathbf{f}}
def bfE{mathbf{E}}
def bfP{mathbf{P}}
def bfa{mathbf{a}}
def bfsig{bm{sigma}}
def bfb{mathbf{b}}
def bfepsilon{bm{e}}
def ev{mathbb{E}}
def sign{textrm{sign}}
def pr{mathbb{P}}
def bfW{mathbf{W}}
def bff{mathbf{f}}
def bfw{mathbf{w}}
def bfA{mathbf{A}}
def bfPsi{mathbf{Psi}}
def bft{mathbf{t}}
def bfv{mathbf{v}}
def bfu{mathbf{u}}
def bfP{mathbf{P}}
def bfR{mathbf{R}}
def cid{xrightarrow[text{}]{text{$mathbb{L}$}}}
def cip{xrightarrow[text{}]{text{$mathbb{P}$}}}
def cae{xrightarrow[text{}]{text{$a.s.$}}}
newcommand{vo}{vec{o}@ifnextchar{^}{,}{}}
newcommand{ip}[1]{langle #1 rangle}
newcommand{floor}[1]{leftlfloor #1 rightrfloor}
%newcommand{ceil}[1]{leftlceil #1 rightrceil}


usepackage{fontspec}
setmainfont{Times New Roman}

RequirePackage{amsthm,amsmath,amsfonts,amssymb}
RequirePackage[]{natbib}
%RequirePackage{unicode-math}
RequirePackage{graphicx,enumitem,comment}
%allowdisplaybreaks 
%
usepackage{geometry}
geometry{ margin=1in}
% In your preamble
usepackage{xr-hyper}
RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

%usepackage{unicode-math}
%setmathfont{XITS Math}
%myexternaldocument{Spatial-SIR-Suppl}

usepackage{multirow}

%
usepackage{bm}
usepackage[dvipsnames]{xcolor}
usepackage{mathrsfs}

startlocaldefs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% Uncomment next line to change            %%
%% the type of equation numbering           %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%numberwithin{equation}{section}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% For Axiom, Claim, Corollary, Hypothesis, %%
%% Lemma, Theorem, Proposition              %%
%% use theoremstyle{plain}                 %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%theoremstyle{plain}

newtheorem{axiom}{Axiom}
newtheorem{claim}[axiom]{Claim}
newtheorem{theorem}{Theorem}[section]
newtheorem{lemma}{Lemma}[section]
newtheorem{corollary}{Corollary}[section]
newtheorem{proposition}{Proposition}[section]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%% For Assumption, Definition, Example,     %%
%% Notation, Property, Remark, Fact         %%
%% use theoremstyle{remark}                %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
theoremstyle{remark}
newtheorem{remark}{Remark}
newtheorem{definition}[theorem]{Definition}
newtheorem{example}{Example}
newtheorem{fact}{Fact}
newtheorem{assumption}{}
renewcommandtheassumption{(Carabic{assumption})}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Please put your definitions here        %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

endlocaldefs

